Pushing the Limit of Range Resolution Beyond Bandwidth Constraint with Triangle FMCW

This paper proposes a novel signal processing technique that doubles the range resolution of FMCW~(Frequency Modulated Continuous Wave) sensing without increasing the required bandwidth. The proposed design overcomes the resolution limit imposed by bandwidth by exploiting the phase consistency observed in the special frequency variation of the beat signal derived from triangle FMCW. Through this approach, the resolution is doubled while maintaining high spectrum SNR. A system model for signal processing is presented, and the energy distribution of the derived beat spectrum is analyzed. The effectiveness of the proposed technique is validated through model-based simulations.

==> 2-SignalModel.tex <==
\section{FMCW Based Ranging} 
\label{sec:signal_model}

%We model the process of FMCW based ranging in this section.
The general form of modulated baseband signal is given as below,
\begin{equation}
	\label{e:tx_bb}
	x(t) = A e^{j \phi (t)}
\end{equation}
where $A$ represents the amplitude, and $\phi (t)$ denotes the time varying signal phase. 
For conventional linear FMCW as shown in Fig.~\ref{f:waveform_tri_ext}~(b), the frequency increases linearly with time, 
which can be formulated as $f(t)=kt+f_{0}$ where $f_{0}$ denotes the starting frequency and $k$ represents the slope that equals the ratio of bandwidth~($B$) to chirp duration~($T_c$) which describes the speed of frequency increase.
The signal phase at time $t$ equals the integral of the varying frequency over time (assuming the initial phase is calibrated to zero),
\begin{equation}
	\label{e:tx_bb_phase}
	\phi (t) = \int_{0}^{t} {2 \pi (kt+f_{0}) d \tau} = \pi k t^2 + 2 \pi f_{0} t
\end{equation}
The baseband signal will be up-converted, transmitted for channel sampling, and received after certain time delay.
The received baseband signal can be formulated as below:
\begin{equation}
	\label{e:rx_bb}
	y(t) = A^{\prime}e^{j \phi (t - \tau)}
\end{equation}
where $A^{\prime}$ and $\tau$ represent the amplitude and time delay of the received signal.
%
The signal is mixed with the conjugate of the original reference signal to derive the beat signal as below,
\begin{equation}
	\label{e:rx_IF}
	y_{beat}(t) = \overline{x(t)} \cdot y(t) = A e^{-j \phi (t)} \cdot A^{\prime}e^{j \phi (t - \tau)}
\end{equation}
By incorporating Eq.~\ref{e:tx_bb_phase}, the formulation of $y_{beat}(t)$ can be reduced to
\vspace{-1mm}
\begin{equation}
	\label{e:rx_IF_reduced}
	y_{beat}(t) = A A^{\prime} e^{j (-2 \pi k \tau t + \pi k {\tau^2} - 2 \pi f_{0} \tau)}
	\vspace{-1mm}
\end{equation}
The beat signal derived from Eq.~\ref{e:rx_IF_reduced} is a single tone oscillating at the frequency of $k\tau$, which can be identified from the beat spectrum derived from FFT. 

%% \vspace{3pt}\noindent\textbf{Time resolution of the beat spectrum.} 
The time resolution is thus determined by the frequency resolution of the derived beat spectrum. 
In FFT, the frequency resolution of a signal segment equals to the inverse of its duration. 
Therefore, for the beat spectrum derived with the FMCW of length $T_c$, the frequency resolution is $1/T_c$, which is mapped to the time resolution of $1/(kT_c)$. 
For conventional linear FMCW with $B=kT_c$, the expression of the time resolution can be simplified to $1/B$ as most widely recognized. 
The time resolution determines the ranging resolution as the distance is measured as the product of signal propagation speed and transmission delay. 

==> 4-MathProof.tex <==
\section{Proof of Phase Consistency}
\label{sec:mathProof}

As we described in the previous section, the real part of the derived beat signal exhibits an important time domain characteristic of phase consistency. We prove the correctness of this observation in this section. 

As shown in Fig.~1, one triangle-FMCW symbol contains a linear chirp and its own mirror. We model the triangle-FMCW with the following piecewise function (assume normalized amplitude),
%
\begin{equation}
    x_{tri}(t)=
    \begin{cases} 
      e^{j (\pi k t^2 + 2\pi f_0 t) }, & 0 < t \leq T_c \\
      e^{j [\phi (T_c) - \pi k t^2 + 2\pi (f_0+B) t] }, & T_c < x \leq T_s
   \end{cases}
   \label{eq:1}
\end{equation}
%
where $B$ is the bandwidth, $T_s$ is the duration of one symbol, and $T_c = Ts/2$ is the duration of a single chirp. Given $f_0=0$, the phase at time $T_c$ is as follows,
%
\begin{equation}
    \phi (T_c) = \pi k {T_c}^2 = \pi B T_c
    \label{eq:2}
\end{equation}
%
By substituting Eq.~\ref{eq:2} to Eq.~\ref{eq:1}, we can simplify the model of one triangle-FMCW symbol as follows,
%
\begin{equation}
    x_{tri}(t)=
    \begin{cases} 
      e^{j (\pi k t^2) }, & 0 < t \leq T_c \\
      e^{j \pi [2 B(t-T_c) - k (t-T_c)^2] }, & T_c < x \leq T_s
   \end{cases}
   \label{eq:3}
\end{equation}
%
The signal is transmitted and gets reflected by the target object. The received signal is a delayed version of the transmitted signal, i.e., $y_{tri}(t)=x_{tri}(t-\tau)$. Specifically,
%
\begin{equation}
    y_{tri}(t)=
    \begin{cases}
      0, & 0 < t \leq \tau \\
      e^{j [\pi k (t-\tau)^2] }, & \tau < t \leq T_c + \tau \\
      e^{j \pi [2 B(t-T_c-\tau) - k (t-T_c-\tau)^2] }, & T_c + \tau < x \leq T_s
   \end{cases}
   \label{eq:4}
\end{equation}
%
To estimate the delay, we produce the beat signal with triangle-FMCW in the same way as Eq.~\ref{e:tx_bb} illustrates,
%
\begin{equation}
    y_{b}(t) = \overline{x_{tri}(t)} \cdot y_{tri}(t)
    \label{eq:5}
\end{equation}
%
The beat signal derived with Eq.~\ref{eq:5} contains the three segments as shown in Fig.~\ref{f:IQ}~(a). 
From time $\tau$ to $T_c$~(i.e., segment~\circled{1}), both $x_{tri}(t)$ and $y_{tri}(t)$ are with the increasing frequency, therefore,
%
\begin{equation}
    y_{b}(t) = e^{-j \pi k t^2} \cdot e^{j \pi k (t-\tau)^2}, \tau < t \leq T_c
    \label{eq:S1}
\end{equation}
%
Similarly, we derive the expression of segment \circled{2} and \circled{3} by multiplying the corresponding part of $\overline{x_{tri}(t)}$ and $y_{tri}(t)$. 
Finally, the beat signal can be formulated as below,
%
\begin{equation}
    y_{b}(t)=
    \begin{cases}
        e^{j \pi (-2k\tau t + k {\tau}^2)}, & \tau < t \leq T_c \\
        e^{j \pi [2k t^2 - (4 B + 2 k \tau )t + 3 B T_c + k{\tau}^2 ]} , & T_c < t \leq T_c + \tau \\
        e^{j \pi (2k\tau t - 4B\tau - k{\tau}^2)} , & T_c+\tau < t \leq T_s
    \end{cases}
    \label{eq:6}
\end{equation}
%
We analyse the phase variation of the beat signal as below:
\begin{itemize}
    \item From time $\tau$ to $T_c$, the expression of $y_b(t)$ in Eq.~\ref{eq:6} is exactly the same as that in Eq.~\ref{e:rx_IF_reduced}, and thus the beat signal obtained with triangle-FMCW is in phase with that derived from extended FMCW during segment \circled{1}.
    \item During $T_c$ to $T_c+\tau$, the phase rotates with a varying speed due to the frequency variation, and is misaligned with the single tone. We analyse the impact of the phase misalignment in Sect.~\ref{sec:simulation}.
    \item From $T_c+\tau$ to $T_s$, $y_b(t)$ is the conjugate of the single tone in Eq.~\ref{e:rx_IF_reduced} when $e^{-j 4 \pi B \tau} = 1$, i.e., $\tau = k/{2B}, k~\in~\mathbb{N}$. Therefore, at the granularity~(i.e., $1/{2B}$) that extended-FMCW can accurately measure, the phase of the real part beat signal, i.e., $\operatorname{Re}[y_b(t)]$ is well aligned with that obtained with extended-FMCW. 
\end{itemize}
%
In summary, the phase of the beat signal obtained with triangle-FMCW is synchronized with the single tone provided by extended-FMCW during segment~\circled{1}. The two beat signals are also aligned in phase of their real part during segment~\circled{3}. The theoretical analysis 
explains the simulation result shown in Fig.~\ref{f:IQ}, and proves the correctness of our observation on the phase consistency.

==> 5-Simulation.tex <==
% \vspace{-3mm}

\section{Evaluation}
\label{sec:evaluation}

% \vspace{-1mm}

In this section, we adopt simulation and real-world experiment to demonstrate the effectiveness of the proposed method by comparing its ranging resolution with those obtained from other approaches as listed below: 
1) using the same triangle FMCW but adopting a different processing method~\cite{li2015method} (referred to as triangle FMCW-Li)
2)~adopting our proposed processing method but using sawtooth FMCW
and 3) adopting our method but using gentle FMCW.
The spectrograms of sawtooth and gentle FMCW are as presented in Fig.~\ref{f:waveforms}.

% In this section, we evaluate the efficacy of using triangle FMCW for improved range resolution with both model based simulation as well as real-world experiment.
%We first validate the improvement with simulation, and then conduct experiment to prove the efficacy with real world acoustic channel. 
%We first simulate the performance provided by triangle FMCW, with reference to that obtained with linear FMCW that uses twice the bandwidth. We then conduct experiment that validates the efficacy with real world acoustic and RF channel. 

%We first benchmark the performance provided by triangle-FMCW against the reference obtained with extended-FMCW,
%We also compare the result with two other naive options
%that expands the same duration but does not produce \textit{phase consistency}.
%and then assess the impact of the path delay~(i.e., $\tau$) on the SNR of the derived beat spectrum. 
%%
% We ask the question that \textit{can we extend the duration of FMCW symbol without increasing the bandwidth?} To achieve so, we have three options -- 1) reducing the slope of normal FMCW symbol~(i.e., gentle-FMCW) 
% 2) repeating FMCW symbol sequentially~(i.e., sawtooth-FMCW) 
% and~3)~mirroring FMCW symbol over time~(i.e., triangle-FMCW). 
% To investigate the efficacy of the three waveforms, we firstly conduct a simulation that compares the time resolution provided by the three waveforms, which suggests that the triangle waveform achieves the same resolution as provided by conventional linear FMCW occupying twice the bandwidth. 
%
%\begin{figure*}[t]
%	\centering
%	\begin{minipage}{0.995\textwidth}
%		\centerline{\includegraphics[width=\textwidth]{./figure/fig_waveforms_v2.pdf}}
%	\end{minipage}
%	\vspace{-1mm}
%	\caption{The four waveforms of FMCW: (a) Extended-FMCW (b) Gentle-FMCW (c) Sawtooth-FMCW and (c) Triangle-FMCW. We adopt extended-FMCW using twice the bandwidth to provide the benchmark to compare with.}
%	\vspace{-2mm}
%	\label{f:waveforms}
%\end{figure*}
%
% \vspace{3pt}\noindent\textbf{Time resolution of triangle-FMCW.} 
% As Eq.~\ref{e:rx_IF_reduced} indicates, the multipath components with different delays produce the beat signal that is composed of certain frequencies~(i.e.,~$f_i=k\tau_i$). The minimum separable path delay difference~(i.e.,~time~resolution) maps directly to the frequency resolution of the beat spectrum. We examine the resolution provided by the three waveforms by comparing the derived beat spectrums, with reference to the benchmark produced by normal linear FMCW symbol using twice the bandwidth (i.e., extended-FMCW). 
%

% \begin{figure}
% 	\centering	
% 	\subfloat{{\includegraphics[trim={0mm 0mm 0mm 0mm},clip, width=0.23\textwidth]{./figure/fig_ray3.pdf}}}
% 	\hspace{0.5mm}
% 	\subfloat{{\includegraphics[trim={0mm 0mm 0mm 0mm},clip, width=0.23\textwidth]{./figure/fig_rician3.pdf}}}
% 	\vspace{-1mm}
% 	\caption{The beat spectrum traces derived from triangle and linear FMCW (with twice the bandwidth) with (a) a three-tap Rayleigh and (b) a four-tap Rician multipath channel.}
% 	\label{f:resolution_benchmark}
% 	\vspace{-3mm}
% \end{figure}

\vspace{-5mm}
\subsection{Simulation}
\label{subs:simulation}
\vspace{-1mm}

We send the variations of FMCW waveforms over a four-tap Rayleigh channel where the multipath profile 
% (which represents the delay and attenuation of multiple signal paths) 
can be self defined. 
The received signals 
% (output of the channel model) 
are processed with the four methods to derive separate range profiles which depict the distribution of multipath components at different ranges. 
% The range resolution is represented by the minimum separable path delay difference. 

% Fig.~\ref{f:simu_range} compares the derived range profiles.
% The profile obtained with our proposed method (Fig.~\ref{f:simu_range}a) exhibits three spikes at the range of 53cm, 54cm and 60cm, which accurately maps to the ground-truth ranges (as annotated by the red lines). 
% In Fig.~\ref{f:simu_range}b, although the ground-truth ranges are also identifiable, the profile is polluted by strong side-lobes which are due to the lack of processing on the phase discontinuity. 

% When examining the range resolution, the profiles in Fig.~\ref{f:simu_range}a and Fig.~\ref{f:simu_range}b exhibit 1cm resolution while the other two profiles provide 2cm resolution. 
% % The reason for sawtooth FMCW is that the DFT of two repeated signal snapshots (as illustrated in Fig.~\ref{f:beat_real}) does not improve the frequency resolution over that of one snapshot.
% % (the power of the omitted spikes (e.g., spike at range 50cm) is lower than -70dB). 
% % Although sawtooth and gentle FMCW also double the symbol duration of a single chirp, the two waveforms cannot provide higher resolution beyond the bandwidth limit because of the periodicity property of DFT~\cite{proakis2007digital} and the reduced slope of gentle FMCW~\cite{enwiki:1027754964}, respectively. 
% Although sawtooth and gentle FMCW also double the symbol duration of a single chirp, the two waveforms cannot provide higher resolution beyond the bandwidth limit.
% For sawtooth FMCW, the reason is that the DFT of two repeated signal snapshots actually does not provide better frequency resolution than the DFT of one snapshot due to the periodicity property of DFT~\cite{proakis2007digital}.
% For gentle FMCW, the reason is because the slope of this waveform is reduced by half and thus the width of one frequency bin maps to larger path length difference~\cite{enwiki:1027754964}. 

Fig.~\ref{f:simu_range3} demonstrates the range profiles obtained with the four different FMCW waveforms. 
With the profile obtained from triangle FMCW (Fig.~\ref{f:simu_range3}a), we can clearly distinguish the four paths at the ranges of 51cm, 53cm, 59cm, and 60cm (with a minimum separable range difference of 1cm). The path range estimations are well aligned with the ground-truth (annotated with the vertical red lines). 
Fig.~\ref{f:simu_range3}b presents the results obtained with triangle FMCW-Li, which fails to reflect the correct number of multipath components, and cannot provide sufficient range resolution to resolve the third and fourth path (the two paths merge into the peak formed by their continuous side-lobes). 
Fig.~\ref{f:simu_range3}c depicts the profile obtained with sawtooth FMCW. 
% It can be observed that the two paths with a range difference of 2cm (the first and second paths) can be detected in this result. However, the fourth path is unresolvable due to its close proximity (1cm range difference) to the third path. 
Similarly it fails to resolve the third and forth paths when they are close (1cm range difference).
Fig.~\ref{f:simu_range3}d shows the profile obtained with gentle FMCW. The granularity of this profile coarser (half range granularity) because the slope of gentle FMCW is half of the other waveforms. As a result its resolution of this result cannot exceed 2cm. 
Overall, the range profile obtained with the triangle FMCW provides twice the range resolution compared to the other results.

% Fig. 3 presents how the spectrum $\rm SN_{T}R$ ($\rm N_T$ denotes the spectrum noise induced by the transition period) varies with increasing path delay. 
% The result is obtained with a simulation where a triangle FMCW signal is sent over a single-tap channel. 
% We measure the spectrum $\rm SN_{T}R$ as the channel delay increases.
% As we see from Fig. 3, although the spectrum $\rm SN_{T}R$ reduces with increasing delay, it is still over -7.4~dB~(the spike can still be detected at this $\rm SN_{T}R$) when the delay exceeds 40\% of the chirp duration,
% % (typically tens of micro-seconds)
% which equivalently supports km-level target range for radio frequency based sensing applications. 
% % Next, we further explain the underlying reason for this superiority. 
% %The reason is detailed in Sec.~\ref{subsec:phase}. 
% %The approximation is obtained with the assumption of $T_c \gg \tau$,
% %we analyse the impact of $\tau$ in Sec~\ref{subsec:tau}. 
% % In the rest of this section, we demonstrate the reason of the above observation in Sec.~\ref{subsec:phase}, and analyse the impact of $\tau$ in Sec.~\ref{subsec:tau}.

The presence of the frequency varying segment raises~the noise floor of the beat spectrum and the impact may intensify as target range increases. 
We conduct a further simulation to assess how the increasing range impacts on the spectrum $\rm SN_{T}R$~($\rm N_T$ denotes the spectrum noise induced by the transition period). 
Specifically, a triangle FMCW signal is sent over a single-tap channel model where the path delay increases. 
%We increase the path delay and record the SNR of each test. Fig.~\ref{f:spectrum_SNR} plots the SNR variation with increasing path delay~(normalized to one chirp length). 
We record the $\rm SN_{T}R$ of each measurement and the result is depicted in Fig.~\ref{f:spectrum_SNR}. 
Although $\rm SN_{T}R$ reduces with increasing range, 
% it is still over -7.4~dB~(the spike can still be detected at this $\rm SN_{T}R$) when the range exceeds 12m, which is sufficient for most applications. 
it is still over -7.4~dB~(the spike can still be detected at this $\rm SN_{T}R$) when the delay exceeds 40\% of the chirp duration,
which equivalently supports km-level target range for radio frequency based sensing applications. 

\vspace{-1mm}
\begin{figure*}[t]
	\centering
	\begin{minipage}{0.27\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_eva_simu-tri3.pdf}}
		\vspace{-1mm}
		\subcaption{triangle FMCW}
		\vspace{-1.5mm}		
	\end{minipage}
	%	\hspace{1mm}
	\begin{minipage}{0.23\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_eva_simu-tri-li3.pdf}}
		\vspace{-1mm}
		\subcaption{triangle FMCW-Li}
		\vspace{-1.5mm}		
	\end{minipage}
	% 	\hspace{1mm}
	\begin{minipage}{0.23\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_eva_simu-saw3.pdf}}
		\vspace{-1mm}
		\subcaption{sawtooth FMCW}
		\vspace{-1.5mm}		
	\end{minipage}
	\begin{minipage}{0.23\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_eva_simu-gen3.pdf}}
		\vspace{-1mm}
		\subcaption{gentle FMCW}
		\vspace{-1.5mm}		
	\end{minipage}
	% \vspace{-1mm}
	\caption{The range profiles which depict the distribution of multipath at different ranges that are obtained with the four methods. 
    We break the y axis of (c) to preserve the samples of very low power.
    % The power of the omitted sampling points in (c) is lower than -70dB. 
    % The granularity of the profile in (d) is two times less than the other three profiles. 
    The ground-truth ranges are annotated with red lines.}
	\vspace{-4mm}
	\label{f:simu_range3}
\end{figure*}
%
\begin{figure*}[t]
	\centering
	\begin{minipage}{0.27\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_spacing_tri.pdf}}
		\vspace{-1mm}
		\subcaption{triangle FMCW}
		\vspace{-1.5mm}		
	\end{minipage}
	%	\hspace{1mm}
	\begin{minipage}{0.23\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_spacing_tri-li.pdf}}
		\vspace{-1mm}
		\subcaption{triangle FMCW-Li}
		\vspace{-1.5mm}		
	\end{minipage}
	% 	\hspace{1mm}
	\begin{minipage}{0.23\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_spacing_saw.pdf}}
		\vspace{-1mm}
		\subcaption{sawtooth FMCW}
		\vspace{-1.5mm}		
	\end{minipage}
	\begin{minipage}{0.23\textwidth}
		\centerline{\includegraphics[width=\textwidth]{./figure/fig_spacing_gen.pdf}}
		\vspace{-1mm}
		\subcaption{gentle FMCW}
		\vspace{-1.5mm}		
	\end{minipage}
	% \vspace{-1mm}
	\caption{The measurement results of the spacing between the two reflectors obtained from the four methods. The gound-truth variation of the spacing is annotated with the red lines.}
	\vspace{-7mm}
	\label{f:spacing}
\end{figure*}
%

% \subsubsection{Impact of path delay}
% \label{sec:tau_impact}
%
%According to the analysis in Sec.~\ref{sec:time_resolution}, the ranging accuracy of the proposed method reduces with increasing path delay. 
%The reason is that, the increased path delay results in extended frequency increasing part (i.e., segment \circled{2} of fig.~\ref{f:spectrogram_beat}) of the beat signal, which further translates to rised noise level of the derived beat spectrum. 
%Eq.~\ref{eqa:18} quantifies the variation of the spectrum SNR with increasing path length. 

% The presence of the frequency varying segment raises the noise of the beat spectrum and negatively impact the performance when target range increases. 
% We conduct a further simulation to assess how the increasing range impacts the spectrum $\rm SN_{T}R$~($\rm N_T$ denotes the spectrum noise induced by the transition period). 
% Specifically, a triangle FMCW signal is sent over a single-tap channel where the path length increases over 12m. 
% %We increase the path delay and record the SNR of each test. Fig.~\ref{f:spectrum_SNR} plots the SNR variation with increasing path delay~(normalized to one chirp length).
% We record the $\rm SN_{T}R$ of each measurement and the result is depicted in Fig.~\ref{f:spectrum_SNR}.  
% Although $\rm SN_{T}R$ reduces with increasing range, it is still over -7.4~dB~(the spike can still be detected at this $\rm SN_{T}R$) when the range exceeds 12m, which is sufficient for most applications. 
% % When the delay approaches 40\% of the chirp length, the SNR is~$-7.4$~dB. Though negative, the SNR still represents a strong beat frequency that can be accurately detected (as illustrated in the beat spectrum in Fig~\ref{f:spectrum_SNR}). 
% % The SNR measurements of this simulation conform well with the theoretical predictions~(labeled with red triangles in Fig.~\ref{f:spectrum_SNR}) obtained with Eq.~\ref{eqa:18}. 

\begin{figure}[t]
	\centering
	% \includegraphics[width=0.479\textwidth]{./figure/fig_exp_setup_v2.pdf}
        \includegraphics[width=0.479\textwidth]{./figure/exp_setup3.pdf}
	\caption{The hardware and setup of the real-world experiment.}
	\label{f:exp_setup}
	\vspace{-6mm}
\end{figure}

\vspace{-3mm}
\subsection{Real-world experiment}
%
% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.23\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{./figure/fig_spacing_tri.pdf}
%          \caption{test}
%          \label{fig:tri-FMCW}
%          \vspace{3mm}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.21\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{./figure/fig_spacing_tri-li.pdf}
%          \caption{test}
%          \label{fig:beat_tri-FMCW}
%      \end{subfigure}
%     \caption{test}
%     \label{fig:spacing}
% \end{figure}
%
We conduct real-world experiment to validate the resolution improvement of the proposed approach with a practical acoustic channel. The experiment is detailed as follows. 

% \subsubsection{Experiment setup} Fig.~\ref{f:exp_setup} illustrates the experiment hardware and setup. We use commercial off-the-shelf acoustic interfaces which include a speaker and a four-microphone linear array (only one microphone is used for this experiment) to transmit and receive the signal for channel sampling. Two metal reflectors are placed facing the transceiver at different distances to create reflected paths with different delays. 

% \subsubsection{Methodology}
% The experiment compares the resolvability of the signals reflected from the two targets obtained with the four aforementioned approaches by applying each method
% % The comparison focuses on the range resolution which is determined by the minimum separable path delay difference. 
% to estimate the spacing~(i.e., $\rm \Delta d$ as illustrated in Fig.~\ref{f:exp_setup}) between the two reflectors.
% Specifically, we fix the location of $\rm R1$ at the distance of 40~cm and vary the distance of $\rm R2$ from 50~cm to 40~cm at the step of 1~cm~(10 test locations in total).
% The closer spacing requires higher range resolution to separate the two reflectors. 
% For each location, each of the four approaches is adopted for separate measurement. 
% All waveforms are transmitted as acoustic signal and the bandwidth is set to 8~kHz.

\subsubsection{Experiment setup and methodology} Fig.~\ref{f:exp_setup} illustrates the experiment setup. We use commercial acoustic speaker and microphone for signal transmission and receiving. Two metal reflectors are placed facing the transceiver at different distances to create reflected paths at different ranges. 

The experiment compares the resolvability of the signals reflected from the two targets obtained with the four aforementioned approaches by applying each method
% The comparison focuses on the range resolution which is determined by the minimum separable path delay difference. 
to estimate the spacing~(i.e., $\rm \Delta d$ as illustrated in Fig.~\ref{f:exp_setup}) between the two reflectors. 
Specifically, the location of $\rm R1$ is fixed at the range of 40cm and the range of 
$\rm R2$ is varied from 50cm to 40cm at the step of 1cm.
% The closer spacing requires higher range resolution to separate the two reflectors. 
For each location, each of the four approaches is adopted for separate measurement. 
All waveforms are sent as acoustic signal with 8kHz bandwidth. 

% In this way, we construct the wireless channel dominated by the two reflected paths. 
% For each measurement, we transmit 45 consecutive linear/triangle FMCW symbols for channel sampling and the post-processing averages the results obtained from all symbols.
% We compare the ranging results of the two reflectors with the ground truth to illustrate the improvement on both accuracy and resolution. 
% % and examine the distribution of the ranging error. 



\subsubsection{Result}
Fig.~\ref{f:spacing} compares the spacing results obtained from the four approaches. 
As we can see, when the spacing between the two reflectors is less than 3cm (test indexed 8, 9, 10), only the results obtained with triangle FMCW are essentially consistent with the ground-truth. 
Specifically, the average spacing errors across these three positions for the four methods are 0.48cm, 1.55cm, 2.96cm, and 3.67cm, corresponding to the results from Fig.~\ref{f:spacing}a to Fig.~\ref{f:spacing}d, respectively.
% The spacing error measured with triangle FMCW-Li is due to the impact of the spectrum side-lobes.
% For sawtooth and gentle FMCW, the error is caused by the common effect of low resolution and spectrum side-lobes -- when the spacing is less than 3cm, the two paths merge into one spike on the derived multipath profile, and thus the position of the first side-lobe is misused to be the range of $\rm R2$. 
The spacing errors measured with the other three approaches are caused by the effect of low resolution and spectrum side-lobes -- when the spacing is less than 3cm, the two paths caused by $\rm R1$ and $\rm R2$ merge into one peak and can hardly be differentiated, in this case the position of the second local maximum is misused to be the range of $\rm R2$. 
Overall, the experiment essentially demonstrates the efficacy of our proposed technique.

% Fig.~\ref{f:exp_result} details the ranging results obtained with traditional linear FMCW (Fig.~\ref{f:exp_result}a) and triangle FMCW (Fig.~\ref{f:exp_result}b). 
% Each figure benchmarks the measurement results of the two reflectors against their corresponding ground-truth distances. 
% By comparing Fig.~\ref{f:exp_result}a and Fig.~\ref{f:exp_result}b, we can observe the improvement of using triangle FMCW on both resolution and accuracy: 
% % First, when comparing the measurement results between the two reflectors, we observe that the minimum separable distance is reduced by ?mm and ?mm for the bandwidth of 8 kHz and 16 kHz, respectively, which proves the enhancement of ranging resolution.
% First, with using linear FMCW, the two paths cannot be separated when their distance is smaller than 38.5~mm, i.e., the unresolvable path length difference is 38.5~mm, which is reduced to 22~mm when triangle FMCW is adopted. Such results prove the enhancement in ranging resolution. 
% Second, when comparing the measurement results of a certain waveform against its ground-truth, we found that the results curve derived with triangle FMCW is always located closer to the ground-truth results which verifies the improvement of ranging accuracy. 
% Overall, the experiment essentially validates the efficacy of our proposed technique. By correctly processing the triangle FMCW, we double the FMCW ranging resolution without requiring extra signal bandwidth. 

% The x-coordinate of each sample represents the ground-truth of a certain distance and the y-coordinate gives the average measurement results. 
% As the results suggest, for the same bandwidth, the measurement obtained with triangle FMCW is closer to the ground truth and gives better distance granularity. 
% For example, when the bandwidth is 8~kHz~(Fig.~\ref{f:exp_result}~(a)), using triangle FMCW can capture the distance variation of 10~mm. 
% In comparison, the results obtained with linear FMCW only provides 21~mm granularity. 
% When the bandwidth increases to 16~kHz~(Fig.~\ref{f:exp_result}~(b)), the results provided by triangle FMCW gives $\sim$5.5~mm ranging resolution. 
%
%\begin{figure}[t]
%	\centering	
%	\subfloat{{\includegraphics[trim={0mm 0mm 0mm 0mm},clip, width=0.238\textwidth]{./figure/fig_exp_result1_v2.pdf}}}
%	\hspace{0.5mm}
%	\subfloat{{\includegraphics[trim={0mm 0mm 0mm 0mm},clip, width=0.238\textwidth]{./figure/fig_exp_result2_v2.pdf}}}
%	\vspace{-1mm}
%	\caption{The comparison between the measured results and ground truth for (a) 8~kHz and (b) 16~kHz FMCW of the two waveforms. The results obtained with triangle FMCW provides higher resolution.}
%	\label{f:exp_result}
%	\vspace{-6mm}
%\end{figure}
% \begin{figure}[t]
% 	\centering
% 	\begin{subfigure}{0.48\textwidth}
% 		\centering
% 		%\includegraphics[width=\textwidth]{./figure/fig_triangleSTFT_annotate.pdf}
% 		\includegraphics[width=\textwidth]{./figure/fig_exp_result_linear.pdf}
% 		\caption{Results obtained with linear FMCW.}
% 	\end{subfigure}
%     \vspace{2mm}
% 	\begin{subfigure}{0.48\textwidth}
% 		\centering
% 		%\includegraphics[width=\textwidth]{./figure/fig_linearSTFT_annotate.pdf}
% 		\includegraphics[width=\textwidth]{./figure/fig_exp_result_triangle.pdf}
% 		\caption{Results obtained with triangle FMCW.}
% 	\end{subfigure}
% 	\vspace{-2mm}
% 	\caption{The ranging results obtained with the two different waveforms which are benchmarked against their corresponding ground truth.}
% 	\label{f:exp_result}
% 	\vspace{-5mm}
% \end{figure}
%
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.459\textwidth]{./figure/fig_exp_cdf_narrow_v2.pdf}
% 	\caption{The CDF of FMCW ranging error of different waveforms and bandwidths. The proposed triangle FMCW based solution approaches the resolution of conventional FMCW with twice the bandwidth.}
% 	\label{f:exp_cdf}
% 	\vspace{-3mm}
% \end{figure}
%

% We further derive the ranging error by calculating the differential between the ground truth and measurement results. The CDF in Fig~\ref{f:exp_cdf} presents the statistical distribution of the ranging errors. 
% For the same bandwidth, the triangle FMCW based processing always provides lower errors. 
% Specifically, for 8~kHz bandwidth, the median error of the linear and triangle FMCW based processing is 4.25~mm and 3.88~mm, respectively. 
% For 16~kHz bandwidth, the median error derived with the two waveforms is 3.88~mm and 3.13~mm.
% When comparing the results across different bandwidth, we see that the median error obtained with 8~kHz triangle FMCW is similar to that provided by 16~kHz linear FMCW. 
% The distribution of the CDF curve suggests that the 8~kHz triangle FMCW provides higher accuracy than the 16~kHz linear FMCW for most of the measurements. 
%Overall, the experiment essentially validates the efficacy of our proposed technique -- by correctly processing the triangle FMCW, we double the FMCW ranging resolution without requiring extra signal bandwidth. 

